Parsing the Switch: LLM-Based UD Annotation for Complex Code-Switched and Low-Resource Languages

Code-switching presents a complex challenge for syntactic analysis, especially in low-resource language settings where annotated data is scarce. While recent work has explored the use of large language models (LLMs) for sequence-level tagging, few approaches systematically investigate how well these models capture syntactic structure in code-switched contexts. Moreover, existing parsers trained on monolingual treebanks often fail to generalize to multilingual and mixed-language input. To address this gap, we introduce the BiLingua Parser, an LLM-based annotation pipeline designed to produce Universal Dependencies (UD) annotations for code-switched text. First, we develop a prompt-based framework for Spanish-English and Spanish-Guaran\'i data, combining few-shot LLM prompting with expert review. Second, we release two annotated datasets, including the first Spanish-Guaran\'i UD-parsed corpus. Third, we conduct a detailed syntactic analysis of switch points across language pairs and communicative contexts. Experimental results show that BiLingua Parser achieves up to 95.29% LAS after expert revision, significantly outperforming prior baselines and multilingual parsers. These results show that LLMs, when carefully guided, can serve as practical tools for bootstrapping syntactic resources in under-resourced, code-switched environments. Data and source code are available at https://github.com/N3mika/ParsingProject

==> tables/analysis_deprel.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lrr}
\toprule
\textbf{DEPREL (Total)} & \textbf{eng→spa} & \textbf{spa→eng} \\
\midrule
nsubj (518)     & 26\% (134)  & 74\% (384)  \\
root (407)      & 40\% (163)  & 60\% (244)  \\
obj (316)       & 25\% (80)   & 75\% (236)  \\
mark (298)      & 68\% (202)  & 32\% (96)   \\
det (258)       & 66\% (170)  & 34\% (88)   \\
case (246)      & 66\% (162)  & 34\% (84)   \\
advmod (242)    & 64\% (155)  & 36\% (87)   \\
obl (150)       & 0\% (-- )   & 100\% (150) \\
cc (106)        & 100\% (106) & 0\% (-- )   \\
discourse (159) & 37\% (59)   & 63\% (100)  \\
iobj (35)       & 100\% (35)  & 0\% (-- )   \\
compound (84)   & 0\% (-- )   & 100\% (84)  \\
\bottomrule
\end{tabular}
\caption{Dependency relation frequencies for English→Spanish and Spanish→English switches. Each row shows the total occurrences in parentheses next to the DEPREL tag, followed by percentage and absolute counts in each direction. Dashes (--) indicate zero occurrences.}
\label{tab:deprel_summary}
\end{table}


==> tables/old_result.tex <==
\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{llllll}
\toprule
\textbf{Study} & \textbf{Languages} & \textbf{POS before} & \textbf{Parsing before} & \textbf{POS after}& \textbf{Parsing after}\\
\midrule
\citet{solorio2014overview} & Spanish--English & 85.1\% & --& -- & --  \\
\citet{solorio2014overview} & Hindi--English   & 83.3\% & --& -- & --  \\
\citet{rijhwani2017analyzing} & Spanish--English & 80.0\% & --& -- & --  \\
\citet{ozates-etal-2022-improving} & Hindi--English & -- & 71.93\% & -- & -- \\
\citet{ozates-etal-2022-improving} & Turkish--German & -- & 73.0\% & -- & -- \\
\citet{bhat-etal-2018-universal} & Hindi--English & -- & 71.03\% & -- & -- \\
%GPT & Spanish--English & 99.54\% & 95.29\% \\
\rowcolor{yellow}
LLM & Spanish--English & 84.21\% & 76.32\% & 99.54\% & 95.29\%\\
\rowcolor{yellow}
LLM & Spanish--Guaraní & 68.38\% & 59.90\% & -- %97.01\% 
& 77.42\%
\\
UDSL & Spanish--English & -- & 47.79\% & -- & -- \\
\bottomrule
\end{tabular}
}
\caption{LLM - and UDSL Performance in POS tagging and dependency parsing according to LAS before and after Human Revision of LLM-based Annotations}
\label{tab:cs_baseline_results}
\end{table}

